Retrospective Analysis of the 2019 MineRL Competition on Sample Efficient Reinforcement Learning

To facilitate research in the direction of sample efficient reinforcement learning, we held the MineRL Competition on Sample Efficient Reinforcement Learning Using Human Priors at the Thirty-third Conference on Neural Information Processing Systems (NeurIPS 2019). The primary goal of this competition was to promote the development of algorithms that use human demonstrations alongside reinforcement learning to reduce the number of samples needed to solve complex, hierarchical, and sparse environments. We describe the competition, outlining the primary challenge, the competition design, and the resources that we provided to the participants. We provide an overview of the top solutions, each of which use deep reinforcement learning and/or imitation learning. We also discuss the impact of our organizational decisions on the competition and future directions for improvement.

==> makejmlrbook <==
#!/usr/bin/env perl
# File          : makejmlrbook
# Author        : Nicola L C Talbot
# Date          : 22nd March 2010
# Last Modified : 30 May 2012
# Version       : 0.32
# Description   : Given the name of a document using the
#                 jmlrbook class file, this script runs
#                 pdflatex (and possibly bibtex) on the
#                 imported articles and the main document.
# http://theoval.cmp.uea.ac.uk/~nlct/
#
# This file is distributed as part of the jmlr LaTeX bundle.
#
# Copyright (c) 2006 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

use Getopt::Long;
use File::Basename;
use File::Copy;
use Cwd;
use strict;

my $version = "0.32 (2012-05-28)";

my $eol = "\n";
my $dd  = '/';

if ($^O eq 'MSWin32')
{
  $eol = "\r\n";
  $dd = "\\";
}

my $showversion      = 0;
my $showhelp         = 0;
my $quiet            = 0;
my $batchtex         = 0;
my $online           = 1;
my $print            = 1;
my $html             = 1;
my $latexapp         = 'pdflatex';
my $bibtexapp        = 'bibtex';
my $latexopts        = '';
my $bibtexopts       = '';
my $format           = 'pdf';
my $logourl          = '';
my $extractpreface   = 0; # v0.3 added
# execute system calls (--noexecute will just list the system calls
# without executing them)
my $execute          = 1; # v0.31 added

unless(&GetOptions(
   "online!"          => \$online,
   "print!"           => \$print,
   "html!"            => \$html,
   "extractpreface!"  => \$extractpreface,
   "logourl=s"        => \$logourl,
   "format=s"         => \$format,
   "latexapp=s"       => \$latexapp,
   "bibtexapp=s"      => \$bibtexapp,
   "latexopts=s"      => \$latexopts,
   "bibtexopts=s"     => \$bibtexopts,
   "quieter!"         => \$quiet,
   "batchtex!"        => \$batchtex,
   "execute!"         => \$execute,
   "version"          => \$showversion,
   "help"             => \$showhelp))
{
   die "Use --help for help\n";
}

my $appname = basename($0);

if ($showhelp)
{
  die "$appname version $version Copyright (c) 2010 Nicola L C Talbot\n",
    "Distributed under the LaTeX Project Public License.\n\n",
    "Syntax: $appname [options] <filename>\n\n",
    "<filename> should be the name of the master document for a LaTeX \n",
    "file that uses the jmlrbook class. The .tex extension may be\n",
    "omitted.\n\n",
    "Basic options:\n",
    "--online\t\tGenerate the color on-line version (default)\n",
    "--noonline\t\tDon't generate the color on-line version\n",
    "--print\t\t\tGenerate the grayscale print version (default)\n",
    "--noprint\t\tDon't generate the grayscale print version\n",
    "--html\t\t\tGenerate the HTML version (default)\n",
    "--nohtml\t\tDon't generate the HTML version\n",
    "--extractpreface\tParse document for preface environment\n",
    "--noextractpreface\tDon't parse document for preface environment\n",
    "--logourl <url>\tMake the logo on the HTML index page link to <url>\n",
    "--batchtex\t\tRun TeX in batch mode\n",
    "--nobatchtex\t\tDon't run TeX in batch mode\n",
    "--quieter\t\tReduce messages to stdout and run TeX in batch mode\n",
    "--noquieter\t\tDon't reduce messages to stdout\n",
    "--execute\t\tExecute system calls (default)\n",
    "--noexecute\t\tDon't execute system calls, just list the\n",
    "\t\t\tcommands.\n",
    "--version\t\tDisplay version number and exit\n",
    "--help\t\t\tDisplay help message and exit\n",
    "\nAdvanced options:\n",
    "--latexapp <name>\tApplication used to call LaTeX\n",
    "\t\t\t(Defaults to 'pdflatex')\n",
    "--format <string>\tOutput format (default: 'pdf')\n",
    "--bibtexapp <name>\tApplication used to call BibTeX\n",
    "\t\t\t(Defaults to 'bibtex')\n",
    "--latexopt <string>\tOptions to pass to LaTeX\n",
    "--bibtexopt <string>\tOptions to pass to BibTeX\n";
}

if ($showversion)
{
  die "$appname version $version copyright (c) 2010 Nicola L C Talbot\n",
    "Distributed under the LaTeX Project Public License.\n";
}

unless ($#ARGV == 0)
{
   die "$appname: missing filename\n",
       "use --help for help\n";
} 

if ($quiet or $batchtex)
{
   $latexopts = '-interaction=batchmode '.$latexopts;
}

if ($quiet)
{
   $bibtexopts = '-terse '.$bibtexopts;
}

my ($main_name, $main_path, $main_suffix) 
  = fileparse($ARGV[0], '\.(tex|ltx)');

$main_suffix = '.tex' unless $main_suffix;

my $org_dir = cwd();

&chdirordie($main_path);

my $mainaux = "$main_name.aux";

# If the aux file doesn't exist or the aux file is older than
# the main file, run latex

if (not -e $mainaux or (-M $mainaux > -M "$main_name$main_suffix"))
{
   &latex($main_name);
}

my $main_bibdata = 0;
my @imports = ();
my %pagerefs = ();
my $preface_data; # v0.3 new
my @preface_editors = ();

# Parse aux file

&parsemainaux($mainaux);

# Replace any instances of \articlepagesref

foreach my $import (@imports)
{
   my $label = $import->{'label'};

   my $pages = $pagerefs{$label}->{'start'}.'--'
             . $pagerefs{$label}->{'end'};

   $import->{'author'}=~s/\\articlepagesref\s*{$label}/$pages/;
}

if ($html)
{
   # If the html files need to be created, make the directory
   # html-src, if it doesn't already exist

   unless (-d 'html-src')
   {
      &mkdirordie('html-src');
   }

   unless (-d 'html')
   {
      &mkdirordie('html');
   }

   if ($extractpreface) # v0.3 new
   {
      # If the preface needs to be extract, make a directory for it if
      # it doesn't already exist

      my $prefdir = &fname("html-src", $preface_data->{'OutFile'});

      unless (-d $prefdir)
      {
         &mkdirordie($prefdir);
      }

      my $prefbase = &fname($prefdir, $preface_data->{'OutFile'});

      &createprefacefile($prefdir, $prefbase);

      # Create the cfg file

      &createjmlrcfg("html-src", $preface_data->{'OutFile'});

      &chdirordie($prefdir);

      &latex($preface_data->{'OutFile'});
      &htlatex($preface_data->{'OutFile'}, 'jmlr');

      &chdirordie($org_dir, $main_path);

      # Check the appropriate subdirectory is in html directory

      my $outname = &fname('html', $preface_data->{'OutFile'});

      unless (-d $outname)
      {
         &mkdirordie($outname);
      }

      # Copy pdf file

      &copyordie("$prefbase.$format",
                &fname($outname, "$preface_data->{OutFile}.$format"));

      # Copy html file

      &copyhtml($preface_data->{'OutFile'}, $preface_data->{'OutFile'});
   }
}

# Iterate through each imported article

foreach my $import (@imports)
{
   my $label = $import->{'label'};
   my $importbase = &fname($import->{'path'}, $import->{'name'});

   # Check the aux file of this article

   my $aux = "$importbase.aux";

   # The aux file should exist because running LaTeX on the
   # main file will create the aux file.

   my $bibdata = 0;

   if (open AUX, $aux)
   {
      &message("Reading '$aux'...\n");

      while (<AUX>)
      {
         if (/\\bibdata\b/)
         {
            $bibdata = 1;
         }
      }
  
      close AUX;
   }
   elsif (not $execute)
   {
      warn "Can't open '$aux' - skipping\n";
   }
   else
   {
      die "$appname: Can't open '$aux' $!\n";
   }

   # Do we need a bibtex run?

   if ($bibdata)
   {
      my $log = "$importbase.log";

      # If the log file doesn't exist, run LaTeX

      unless (-e $log)
      {
         &chdirordie($import->{'path'});

         &latex($import->{'name'});

         &chdirordie($org_dir, $main_path);
      }

      open LOGFD, $log or die "$appname: Can't open '$log' $!\n";

      &message("Reading '$log'...\n");

      my $runbibtex = 0;

      while (<LOGFD>)
      {
         if (/There were undefined citations\./)
         {
            # Run bibtex and latex
            $runbibtex = 1;

            last;
         }
      }

      close LOGFD;

      if ($runbibtex)
      {
         &chdirordie($import->{'path'});

         &bibtex($import->{'name'});
         &latex($import->{'name'});

         &chdirordie($org_dir, $main_path);
      }
   }

   if ($html)
   {
      # If html is required, we also need pdf versions of the
      # individual articles.

      # v0.2 run latex even if pdf file exists to ensure start page 
      # number is correct.

      &chdirordie($import->{'path'});

      &latexstartpage($import->{'name'}, $pagerefs{$label}->{'start'});

      &chdirordie($org_dir, $main_path);

      # Do we need a rerun?

      if (&needs_rerun($importbase))
      {
         &chdirordie($import->{'path'});

         &latexstartpage($import->{'name'}, $pagerefs{$label}->{'start'});

         &chdirordie($org_dir,$main_path);
      }

      my $importdir = $import->{'path'};

      if ($importdir = '.')
      {
         $importdir = $import->{'name'};
      }

      # Check the appropriate subdirectory is in html-src

      my $name = &fname('html-src', $importdir);

      unless (-d $name)
      {
         &mkdirordie($name);
      }

      my $text = '';

      # Read the LaTeX file and store everything up to
      # the end of the abstract

      my $tex = "$importbase.tex";

      my $absfile = &fname("html-src", $importdir,
                           $import->{'name'}.'.tex');

      if ($execute)
      {
         open TEX, $tex or die "$appname: Can't open '$tex': $!\n";

         while (<TEX>)
         {
            # This doesn't handle complicated cases, such as
            # the author using \abstract ... \endabstract
            # or commenting out the abstract with conditionals
            if (/^([^%]*)\\end{abstract}/)
            {
               $text .= $&;
               last;
            }

            $text .= $_;
         }

         close TEX;

         # Add the 'html' class option:
         unless ($text=~
          s/^([^%]*)\\documentclass\s*\[(.*)\]/$1\\documentclass[$2,html]/m)
         {
           $text=~s/^([^%]*)\\documentclass\s*/$1\\documentclass[html]/m;
         }

         my $aux = "$importbase.aux";

         $aux=~s/\\/\//g if ($dd eq '\\');

         my $prebegindoc = '\\hypersetup{draft}' . $eol
                         . '\\makeatletter' . $eol
                         . "\\input{../../$aux}" . $eol
                         . '\\makeatother'
                         . $eol;

         my $begindoc = '';

         # Set the authors
         if (defined($import->{'author'}))
         {
            my $author = $import->{'author'};

            $author=~s/^([^;]*);/\\textbf{\\emph{$1};}/;

            $begindoc .= "\\jmlrauthors{$author}";
         }

         # Add content div

         # v0.31 modified \footnote to set the footnote text as in-line
         # parenthesis.

         $text=~s/^([^%\n\r\f]*)\\begin{document}/
                 $prebegindoc$&$begindoc
                 \\HCode{<div id="content">}
                 \\renewcommand{\\footnote}[2][]{ (\#2)}%$eol
                 /mx;

         # Create file containing the abstract

         open ABSFD,">$absfile" 
           or die "$appname: Can't create '$absfile': $!\n";

         print ABSFD "\\batchmode", $eol if ($batchtex or $quiet);

         my $texpath = $import->{path};

         $texpath=~s/\\/\//g if ($dd eq '\\');

         print ABSFD
           "\\makeatletter",$eol,
           "\\def\\input\@path{{../../$texpath/}}$eol",
           "\\makeatother",$eol,
           $text, $eol, 
           "\\HCode{", &htmltimestamp, "}", $eol,
           "\\HCode{</div>}", $eol,
           &htmlmenu, # v0.3 added by Olivier Chapelle
           "\\end{document}",$eol;

         close ABSFD;
      }
      else
      {
         &messagecall("Skipping creation of '$absfile'\n");
      }

      # Create the cfg file

      &createjmlrcfg("html-src", $importdir);

      # Run htlatex

      # Change directory
      &chdirordie("html-src", $importdir);

      &htlatex($import->{'name'}, 'jmlr');

      # Go back to main directory

      &chdirordie($org_dir, $main_path);

      # Copy the html file to the html directory, but rename
      # the css file to jmlr.css

      &copyhtml($importdir, $import->{'name'});

      # Check the appropriate subdirectory is in html directory

      my $outname = &fname('html', $importdir);

      unless (-d $outname)
      {
         &mkdirordie($outname);
      }

      # Copy pdf file

      &copyordie("$importbase.$format",
                 &fname($outname, "$import->{name}.$format"));
   }
}

# do we need to run bibtex on the main document?

if ($main_bibdata)
{
   &bibtex($main_name);
}

if ($online)
{
   &latexonline($main_name);

   # do we need a rerun?

   if (&needs_rerun($main_name))
   {
      &message("Rerun required\n");
      &latexonline($main_name);

      # check again

      if (&needs_rerun($main_name))
      {
         &message("Rerun required\n");
         &latexonline($main_name);
      }
   }
}

if ($print)
{
   &latexprint($main_name);

   # do we need a rerun?

   if (&needs_rerun($main_name))
   {
      &message("Rerun required\n");
      &latexprint($main_name);

      # check again

     if (&needs_rerun($main_name))
     {
        &message("Rerun required\n");
        &latexprint($main_name);
     }
   }
}

if ($html and $execute)
{
   # Make the index file

   my $indexfile = &fname('html-src', "index");

   my $preamble = '';

   open OUTFD, ">$indexfile.tex" 
    or die "Can't open '$indexfile.tex': $!\n";

   open INFD, "$main_name.tex"
     or die "Can't open '$main_name.tex': $!\n";

   print OUTFD "\\batchmode", $eol if ($batchtex or $quiet);

   print OUTFD
        "\\makeatletter",$eol,
        "\\def\\input\@path{{../}}$eol",
        "\\makeatother",$eol,
        "\\def\\jmlrgrayscale{0}",$eol;

   while (<INFD>)
   {
      unless
        (s/^([^%]*)\\documentclass\s*\[([^\]]*)\]/
           $1\\documentclass[$2,html]/x)
      {
         s/^([^%]*)\\documentclass\s*/$&\[html\]/;
      }

      s/^([^%]*)\\begin{document}/
        \\hypersetup{draft}$eol$&\\HCode{<div id="content">}/x;

      if (/^([^%]*)\\maketitle/)
      {
         $preamble .= join('', $1, "\\maketitle", $eol);
         last;
      }

      $preamble .= $_;
   }

   close INFD;

   # Find the book logo
   if ($preamble
     =~/\\logo\s*(?:\[[^\]]*\])?\s*{(%\s*\n)?\\includegraphics\s*(\[[^\]]*\])?{([^}]*)}}/m)
   {
      my $texpath = $3;
      my $orgtexpath = $texpath;
      $texpath=~s/\//\\/g if ($dd eq "\\");

      my $ext = '';

      if (-e $texpath)
      {
         &copyordie($texpath, 'html');

         &copyordie($texpath, 'html-src');
      }
      elsif (-e "$texpath.png")
      {
         &copyordie("$texpath.png", 'html');

         &copyordie("$texpath.png", 'html-src');

         $ext = '.png';
      }
      elsif (-e "$texpath.jpg")
      {
         &copyordie("$texpath.jpg", 'html');
         &copyordie("$texpath.jpg", 'html-src');

         $ext = '.jpg';
      }
      elsif (-e "$texpath.gif")
      {
         &copyordie("$texpath.gif", 'html');

         &copyordie("$texpath.gif", 'html-src');

         $ext = '.gif';
      }

      my $img = basename($texpath);
      
      if ($logourl)
      {
         $preamble=~s/
                  \\includegraphics(\[[^\]]*\])?{$orgtexpath}/
                  \\href{$logourl}{\\includegraphics${1}{$img$ext}}/mgx;
      }
      else
      {
         $preamble=~s/
                  \\includegraphics(\[[^\]]*\])?{$orgtexpath}/
                  \\includegraphics${1}{$img$ext}/mgx;
      }
   }

   print OUTFD $preamble, $eol;

   # Parse TOC

   my $toc = "$main_name.toc";

   # Add link to preface if required

   if ($extractpreface)
   {
      print OUTFD
         "\\begin{description}\\item[\\normalfont \\prefacename]", $eol;

      print OUTFD "\\textbf{\\emph{\\jmlrabbrnamelist{{",
                  join('},{', @preface_editors),
                  "}}};} ",
                  '\\csname @jmlrabbrvproceedings\\endcsname\\space',
                  '\\csname @jmlrvolume\\endcsname:',
                  $preface_data->{'Start'};

      unless ($preface_data->{'Start'} eq $preface_data->{'End'})
      {
         print OUTFD '--', $preface_data->{'End'};
      }

      print OUTFD ', \\csname @jmlryear\\endcsname\\newline', $eol;

      my $name = $preface_data->{'OutFile'};

      print OUTFD "[\\HCode{<a href=\"$name.html\">html</a>}] ",
                  "[\\HCode{<a href=\"$name/$name.pdf\">pdf</a>}]",
                  $eol;

      print OUTFD "\\end{description}$eol";
   }

   open TOC, $toc or die "Can't open '$toc': $!\n";

   my $idx = 0;

   while (<TOC>)
   {
      if (/^\\tocpart\s*{(.*)}\s*$/)
      {
         print OUTFD "\\begin{center}\\bfseries $1\\end{center}$eol";
      }
      elsif (/\\contentsline\s*{papertitle}{(.*)}{[^{}]*}{[^{}]*}\s*$/)
      {
         # v0.3 Changed by Olivier Chapelle to use description
         # environment instead of paragraph break
         print OUTFD "\\begin{description}\\item[\\normalfont $1]$eol";
      }
      elsif (/\\contentsline\s*{chapterauthor}{(.*)}{[^{}]*}{[^{}]*}\s*$/)
      {
         my $details = $1;
         $details=~s/([^;]*);/\\textbf{\\emph{$1};}/;

         my $label = $imports[$idx]->{'label'};
         my $pages = $pagerefs{$label}->{'start'}.'--'
                   . $pagerefs{$label}->{'end'};

         $details=~s/\\articlepagesref\s*{$label}/$pages/;

         # v0.3 Changed by Olivier Chapelle to use newline instead of par
         print OUTFD "$details\\newline$eol";

         my $name = $imports[$idx]->{'name'};

         print OUTFD "[\\HCode{<a href=\"$name.html\">abs</a>}] ",
                     "[\\HCode{<a href=\"$name/$name.pdf\">pdf</a>}]",
                     $eol;

         # v0.3 Changed by Olivier Chapelle to end description
         print OUTFD "\\end{description}$eol";

         $idx++;
      }
   }

   close TOC;

   # version 0.2 added time stamp

   print OUTFD "\\HCode{", &htmltimestamp, "}$eol";

   print OUTFD &htmlmenu; # v0.3 Added by Olivier Chapelle

   print OUTFD "\\HCode{</div>}\\end{document}$eol";

   close OUTFD;

   # Go into html-src directory and run htlatex

   &chdirordie('html-src');

   &htlatex("index", 'xhtml');

   &chdirordie('..');

   # Copy to html directory

   my $inname = &fname('html-src', 'index.html');
   my $outname = &fname('html', 'index.html');

   open INFD, $inname or die "Can't open '$inname': $!\n";

   open OUTFD, ">$outname" or die "Can't open '$outname': $!\n";

   while (<INFD>)
   {
      s/href="index.css"/href="jmlr.css"/;

      print OUTFD;
   }

   close OUTFD;

   close INFD;

   # v0.2 new:
   # Copy any images generated by htlatex to html/

   my @imagefiles = glob(&fname('html-src', "index*.png"));

   foreach my $imagefile (@imagefiles)
   {
      copy($imagefile, 'html');
   }
}
elsif ($html)
{
   &messagecall("chdir 'html-src'\n");
   &htlatex("index", 'xhtml');
}

# Return to original directory
chdir $org_dir;

# Subroutines

sub message{ print @_ unless ($quiet) }

sub messagecall{ print @_ if (not $quiet or not $execute) }

sub systemcall{
  my $cmd = shift;

  &messagecall($cmd, "\n");

  my $code = 0;

  $code = system($cmd) if ($execute);

  $code;
}

sub latex{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts, "\"$file\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }
}

# v0.2 new
sub latexstartpage{
   my $file = shift;
   my $page = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\startpage{$page}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }
}

sub copyordie{
   my ($org, $dest) = @_;

   &messagecall("copy '$org' to '$dest'\n");

   if ($execute)
   {
      copy($org, $dest) or die "Can't copy '$org' to '$dest': $!\n";
   }
}

sub latexonline{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\jmlrgrayscale{0}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }

   &copyordie("$file.$format", "$file-online.$format");
}

sub latexprint{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\jmlrgrayscale{1}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }

   &copyordie("$file.$format", "$file-print.$format");
}

sub bibtex{
   my $file = shift;

   my $code = &systemcall(
                 join(' ', $bibtexapp, $bibtexopts, "\"$file\""));

   if ($code)
   {
      die "**BibTeX run failed with exit code $code.**\n",
          "Check '$file.blg' for details\n";
   }
}

sub needs_rerun{
  my $file = shift;
  my $rerun = 0;

  unless ($execute)
  {
     &messagecall("Skipping rerun check for '$file'\n");
     return 0;
  }

  # Scan log file for rerun message

  my $log = "$file.log";

  # If there's no log file a run is needed
  open LOGFD, $log or return 1;

  while (<LOGFD>)
  {
     if (/Rerun to get cross-references right\./)
     {
        $rerun = 1;
        last;
     }
  }

  close LOGFD;

  return $rerun;
}

sub fname{ join($dd, @_) }

# v0.3 new
sub chdirordie{
  my $dirname = &fname(@_);

  &messagecall("chdir '$dirname'\n");

  unless (chdir $dirname)
  {
     if ($execute)
     {
        die "$appname: Can't change directory to $dirname: $!\n";
     }
     else
     {
        warn "(Can't change directory to '$dirname')\n";
     }
  }
}

# v0.31 new
sub mkdirordie{
  my $dirname = &fname(@_);

  &messagecall("mkdir '$dirname'\n");

  unless (mkdir $dirname)
  {
     if ($execute)
     {
        die "$appname: Can't create directory '$dirname': $!\n";
     }
     else
     {
        warn "(Can't create directory '$dirname')\n";
     }
  }
}

# v0.2 new
sub htmltimestamp{
   my $timestamp = localtime;

   return "<hr><center>Page last modified on $timestamp.</center>";
}

# v0.3 Added by Olivier Chapelle
sub htmlmenu{
  return '
\\HCode{<div id="fixed"><br>}
\\HCode{<a align="right" href="http://www.jmlr.org" target=_top><img align="right" class="jmlr" src="http://jmlr.csail.mit.edu/jmlr.jpg" border="0"></a>}
\\HCode{<p><br><br>}
\\HCode{<p align="right"> <A href="http://www.jmlr.org/"> Home Page </A>}
\\HCode{<p align="right"> <A href="/papers"> Papers </A>}
\\HCode{<p align="right"> <A href="/author-info.html"> Submissions </A>}
\\HCode{<p align="right"> <A href="/news.html"> News </A>}
\\HCode{<p align="right"> <A href="/scope.html"> Scope </A>}
\\HCode{<p align="right"> <A href="/editorial-board.html"> Editorial Board </A>}
\\HCode{<p align="right"> <A href="/announcements.html"> Announcements </A>}
\\HCode{<p align="right"> <A href="/proceedings"> Proceedings </A>}
\\HCode{<p align="right"> <A href="/mloss">Open Source Software</A>}
\\HCode{<p align="right"> <A href="/search-jmlr.html"> Search </A>}
\\HCode{<p align="right"> <A href="/manudb"> Login </A></p>}
\\HCode{<br><br>}
\\HCode{<p align="right"> <A href="http://jmlr.csail.mit.edu/jmlr.xml">}
\\HCode{<img src="http://jmlr.csail.mit.edu/RSS.gif" class="rss" alt="RSS Feed">}
\\HCode{</A>}
\\HCode{</div>}
'
}

# v0.3 new
sub htlatex{
   my ($filename, $cfg) = @_;

   # unicode-related options suggested by Olivier Chapelle

   # v0.31 added latex options in 5th parameter

   my $code = &systemcall(join(' ', 'htlatex',
                  "\"$filename\"",
                  "\"$cfg,uni-html4\"",
                  "\" -cunihtf -utf8\"",
                  '""',
                  "\" $latexopts\""
                 ));

   if ($code)
   {
      die "$appname: htlatex failed with exit code $code.\n";
   }
}

#v0.3 new
sub createjmlrcfg{
   my $cfg = &fname(@_, "jmlr.cfg");

   unless ($execute)
   {
      &messagecall("Skipping creation of '$cfg'\n");
      return;
   }

   open CFG, ">$cfg" or die "$appname: Can't create '$cfg': $!\n";

print CFG <<END_CFG;
\\Preamble{html}
\\begin{document}
\\Css{div.maketitle {text-align:left;}}
\\Css{h2.titleHead {text-align:left;}}
\\Css{. {font-family:verdana,helvetica,sans-serif}}
\\Css{a {text-decoration:none;color:\\#3030a0}}
\\Css{.cmbx-10x-x-109{ font-weight: bold;}}
\\Css{.cmbxti-10x-x-109{ font-weight: bold; font-style: italic;}}
\\Css{\\#fixed {position:absolute; top:0; left:0; width:8em;
height:100\\%;}}
\\Css{\\#content {margin-top:1em; margin-left:10em;
margin-right:0.5em;}}
\\Css{img.jmlr {width: 7em;}}
\\Css{img.rss {width: 2em;}}
\\EndPreamble
END_CFG

# v0.3 Last four \Css lines above added by Olivier Chapelle
   close CFG;
}

#v0.3 new
# copy html from html-src/$dir/ to html/ and rename css file
sub copyhtml{
   my ($dir, $name) = @_;

   my $infile = &fname("html-src", $dir, "$name.html");

   my $outfile = &fname("html", "$name.html");

   unless ($execute)
   {
      &messagecall("Copy '$infile' to '$outfile'\n");
      return;
   }

   open INFD, $infile or die "Can't open '$infile': $!\n";

   open OUTFD, ">$outfile" or die "Can't open '$outfile': $!\n";

   while (<INFD>)
   {
      s/href="$name\.css"/href="jmlr.css"/;

      print OUTFD;
   }

   close OUTFD;

   close INFD;

   # Copy css file

   &copyordie("html-src/$dir/$name.css", "html/jmlr.css");
}

sub parsemainaux{
   my $mainaux = shift;

   &message("Reading '$mainaux'...\n");

   unless (open AUX, "$mainaux")
   {
      if ($execute)
      {
         die "$appname: Can't open '$mainaux' $!\n";
      }
      else
      {
         warn "(Can't open '$mainaux' - skipping)\n";
         return;
      }
   }

   while (<AUX>)
   {
      if (/\\bibdata\b/)
      {
         $main_bibdata = 1;
      }
      elsif (/\\\@jmlr\@import{(.*)}{(.*)}{(.*)}/)
      {
         my $import = 
           {
             label => $1,
             path  => $2,
             name  => $3
           };

         $import->{'name'} =~s/\.(tex|ltx)\Z//;

         push @imports, $import;
      }
      elsif (/\\contentsline\s*{chapterauthor}{(.*)}{}{}}\s*$/
        and $#imports > -1)
      {
         $imports[$#imports]->{'author'} = $1;
      }
      elsif (/^\\newlabel\s*{([^}]*)jmlrstart}{{([^}]*)}{([^}]*)}/)
      {
         my $label = $1;
      
         $pagerefs{$label}->{'start'} = $3;
      }
      elsif (/^\\newlabel\s*{([^}]*)jmlrend}{{([^}]*)}{([^}]*)}/)
      {
         my $label = $1;

         $pagerefs{$label}->{'end'} = $3;
      }
      elsif ($extractpreface) # v0.3 new
      {
         if (/^\\\@prefacestart{([^}]*)}{(\d*)}/)
         {
            $preface_data->{'Start'} = $1;
            $preface_data->{'StartArabic'} = $2;
         }
         elsif (/^\\\@prefaceend{([^}]*)}/)
         {
            $preface_data->{'End'} = $1;
         }
         elsif (/^\\\@prefacefile{([^}]*)}{([^}]*)}/)
         {
            $preface_data->{'File'}    = $1;
            $preface_data->{'OutFile'} = $2;
         }
         elsif (/^\\\@prefaceeditor{(.*)}/)
         {
            my $name = $1;
            $name=~s/\\\\.*//;
            push @preface_editors, $name;
         }
      }
   }

   # if preface is to be extracted, has the require data been found?

   if ($extractpreface)
   {
      unless ($preface_data->{'File'})
      {
         warn "$appname: Can't find preface information in aux file.\n",
              "Have you used the preface environment?\n";

         $extractpreface = 0;
      }
   }

   close AUX;
}

sub createprefacefile{
   my ($prefdir, $prefbase) = @_;

   my $prefout = "$prefbase.tex";

   &messagecall("Create preface file '$prefout'\n");

   return unless ($execute);

   # Open preface output file

   open PREFOUT, ">$prefout"
      or die "$appname: Can't open '$prefout': $!\n";

   print PREFOUT "\\batchmode", $eol if ($batchtex or $quiet);
   print PREFOUT "\\makeatletter", $eol;
   print PREFOUT "\\def\\input\@path{{../../}}", $eol;
   print PREFOUT "\\makeatother", $eol;

   # Get the book's preamble

   my $filename = "$main_name$main_suffix";

   open BOOK, $filename
     or die "$appname: Can't open '$filename': $!\n";

   while (<BOOK>)
   {
      if (/\\documentclass/)
      {
         unless (s/^([^%]*)\\documentclass\s*\[(.*)\]/$1\\documentclass[$2,html]/m)
         {
           s/^([^%]*)\\documentclass\s*/$1\\documentclass[html]/m;
         }

         print PREFOUT;
      }
      elsif (/^\\begin{document}/)
      {
         if ($preface_data->{'Start'}=~/^[clxvi]+$/)
         {
            print PREFOUT "\\pagenumbering{roman}%", $eol;
         }
         elsif ($preface_data->{'Start'}=~/^[CLXVI]+$/)
         {
            print PREFOUT "\\pagenumbering{Roman}%", $eol;
         }

         print PREFOUT 
           "\\setcounter{page}{",
           $preface_data->{'StartArabic'},
           "}%", $eol;

         # \hypersetup{draft} is used to suppress links.
         # (Only a partial document so internal links may be
         # dead. Also prevents unwanted tag before the DOCTYPE
         # line in the HTML file.)

         print PREFOUT
               "\\hypersetup{draft}", $eol,
               '\\makeatletter',
               "\\\@openrightfalse\\input{../../$main_name.aux}",
               '\\makeatother', $eol;

         print PREFOUT
               "\\providecommand{\\HCode}[1]{}", $eol,
               "\\title{\\prefacename}", $eol,
               "\\begin{document}", $eol,
               "\\HCode{<div id=\"content\">}", $eol;

         last;
      }
      else
      {
         print PREFOUT;
      }
   }

   close BOOK;

   # Preface file name will have '/' as directory divider

   my $preffile = $preface_data->{'File'};

   if ($dd eq "\\")
   {
      $preffile=~s/\//\\/g;
   }

   open PREFIN, $preffile
     or die "$appname: Can't open '$preffile': $!\n";

   my $scanning  = 0;

   while (<PREFIN>)
   {
      # This is fairly primitive and works best when the begin
      # and end of the environment are on their own line.

      if (/\\begin{preface}/)
      {
         print PREFOUT;
         $scanning = 1;
      }
      elsif ($scanning)
      {
         print PREFOUT;

         last if /\\end{preface}/;
      }
   }

   close PREFIN;

   print PREFOUT
     "\\HCode{", &htmltimestamp, "}", $eol,
     "\\HCode{</div>}", $eol,
     &htmlmenu,
     "\\end{document}", $eol;

   close PREFOUT;

}

1;

